Geography-Aware Self-Supervised Learning

Contrastive learning methods have significantly narrowed the gap between supervised and unsupervised learning on computer vision tasks. In this paper, we explore their application to geo-located datasets, e.g. remote sensing, where unlabeled data is often abundant but labeled data is scarce. We first show that due to their different characteristics, a non-trivial gap persists between contrastive and supervised learning on standard benchmarks. To close the gap, we propose novel training methods that exploit the spatio-temporal structure of remote sensing data. We leverage spatially aligned images over time to construct temporal positive pairs in contrastive learning and geo-location to design pre-text tasks. Our experiments show that our proposed method closes the gap between contrastive and supervised learning on image classification, object detection and semantic segmentation for remote sensing. Moreover, we demonstrate that the proposed method can also be applied to geo-tagged ImageNet images, improving downstream performance on various tasks. Project Webpage can be found at this link geography-aware-ssl.github.io.

==> sections/1_introduction.tex <==
\section{Introduction}

\begin{figure*}[!ht]
\centering
\begin{subfigure}[b]{0.45\textwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/ap1.pdf}
 \label{fig:moco_base}
\end{subfigure}
~
\begin{subfigure}[b]{0.45\textwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/ap2.png}
 \label{fig:moco_ours}
\end{subfigure}
\caption{\textbf{Left} shows the original MoCo-v2~\cite{chen2020improved} framework. \textbf{Right} shows the schematic overview of our approach.}
\label{fig:approach}
\end{figure*}


%Deep learning has demonstrated great success in many computer vision tasks including object detection~\cite{lin2014microsoft,lin2017feature}, image segmentation~\cite{lin2014microsoft,ronneberger2015u}, and image classification~\cite{russakovsky2015imagenet,he2016deep}. 
%\begin{comment}
%Despite recent successes, many modern computer vision methods rely heavily on large-scale labeled datasets, which are often costly and time-consuming to collect~\cite{mahajan2018exploring}. 
Unsupervised learning has recently gained increasing popularity to reduce the dependency on large-scale labeled datasets in computer vision as they are costly~\cite{mahajan2018exploring}. As a result, recent progress in unsupervised learning bridged the gap to supervised learning counterparts on image classification, object detection and semantic segmentation tasks while reducing the dependency on the large-scale labeled datasets~\cite{mahajan2018exploring,grill2020bootstrap,he2020momentum,chen2020improved,chen2020simple}. 
%However, the success of self-supervised and supervised learning methods both require very large-scale datasets~\cite{mahajan2018exploring,miech2020end,he2020momentum}.

One of the most recent unsupervised learning methods, \emph{contrastive learning}~\cite{he2020momentum,chen2020improved,chen2020simple}, has particularly received increasing attention in computer vision community. However, its application to remote sensing images have not been studied yet. We find it surprising since collecting large-scale labeled datasets with remote sensing images are very costly as it requires domain expertise to annotate them~\cite{uzkent2019learning,lam2018xview,christie2018functional}. Inspired by the success of self-supervised learning methods like~\cite{he2020momentum,chen2020improved} and release of large-scale remote sensing datasets~\cite{lam2018xview,christie2018functional,xia2018dota,gupta2019creating}, we explore self-supervised learning on large-scale remote sensing datasets.

%\end{comment}

\begin{comment}
Inspired by the success of self-supervised learning methods ~\cite{he2020momentum,chen2020improved},
%and release of large-scale remote sensing datasets~\cite{lam2018xview,christie2018functional,xia2018dota,gupta2019creating}, 
we explore their application to large-scale remote sensing datasets, e.g. satellite images.
It has been recently shown that self-supervised learning methods perform comparably well or even better than their supervised learning counterpart on image classification, object detection and image segmentation 
on traditional computer vision datasets
%while reducing the dependency on the large-scale labeled datasets
~\cite{mahajan2018exploring,grill2020bootstrap,he2020momentum,chen2020improved,chen2020simple}. However, their application to remote sensing images is largely unexplored, despite the fact that collecting and labeling remote sensing images is  particularly costly as annotations often require domain expertise~\cite{uzkent2019learning,lam2018xview,christie2018functional}.
\end{comment}

% Remote sensing images, on the other hand, are
% particularly challenging to label since they require special understanding on aerial perspectives~\cite{christie2018functional,lam2018xview}. Due to a lack of labeled data, fine grained interpretation of remote sensing images is often hard, hindering the application of remote sensing data in many downstream tasks.~\chenlin{stress that there is a need of finding better ways of understanding remote sensing data without using expensive data. could be a better transition}
% Thus, there is a need of developing algorithms that allow for understanding remote sensing data without expensive labeled data.

% Due to high acquisition cost of high resolution satellite mages\chenlin{labeled?}, up until recently, there was no publicly available large-scale remote sensing datasets.\chenlin{no publicly available large-scale labeled dataset?} Most of the publicly available remote sensing datasets focused on a small geographical area with small number of images representing only a few class categories~\cite{mundhenk2016large,collins2005open,mendoza2009video}. 
% With the increasing amount of publicly  available datasets in many domains, in 2018, three large-scale remote sensing datasets involving image recognition~\cite{christie2018functional} and object detection across the globe have been released to the public~\cite{lam2018xview,xia2018dota}. \chenlin{this paragraph talked too much about datasets. maybe they are not that relevant? we can emphasis more on labeled data is scarce, unlabeled data is abundant. that's why self-supervised learning is useful. the reason we choose the labeled dataset is not because we want to use the label in training, it is because of evaluation.}Inspired by the success of self-supervised contrastive learning methods like~\cite{he2020momentum} in computer vision, we explore self-supervised learning on remote sensing domain where labeled data is usually lacking.

% \chenlin{
% Recent progress in self-supervised contrastive learning has allowed unsupervised learning to perform comparably well or even better than their supervised counterpart on image classification~\cite{he2020momentum,chen2020improved,chen2020simple}, object detection and image segmentation~\cite{he2020momentum,chen2020improved}. 
% Inspired by the success of self-supervised learning methods like~\cite{he2020momentum} on natural images, we explore self-supervised learning on remote sensing data, where unlabeled data is abundant but labeled data is lacking. To the best of our knowledge, no previous work has studied the application of self-supervised learning to remote sensing domain.
% }

% \burak{We can add a paragraph stating that up until recently there was no publicly available large scale remote sensing dataset. With the availability of large-scale dataset, such as fMoW, unsupervised learning on remote sensing datasets can be critical for many downstream tasks etc.}
%Our contribution can be summarized as follows. 
In this direction, we first experimentally evaluate the performance of an existing self-supervised contrastive learning method, MoCo-v2~\cite{he2020momentum} on a remote sensing dataset.
%To the best of our knowledge, no previous work has demonstrated the effectiveness of contrastive learning in the remote sensing domain. 
%While on Imagenet~\cite{deng2009imagenet} MoCo-v2 have considerably reduced the gap with their supervised counterparts, there still exists a reasonable gap. 
We observe that there exists a non-trivial gap between MoCo-v2~\cite{chen2020improved} and supervised learning on a standard remote sensing benchmark~\cite{christie2018functional}. 
\begin{comment}
For instance, on the Functional Map of the World (fMoW) image classification benchmark, we observe an 8\% gap in top 1 accuracy between supervised and self-supervised methods.
% \s{while on imagenet the gap between selfsupervised and supervsied is x, 
% on fwmow we found that the gap between mocov2 and ... is xxx } \ayush{Done.}
We hypothesize that this performance gap could be caused by the highly similar visual content across different classes in remote sensing images. For instance, \emph{single-unit residential} and \emph{office building} are almost indistinguishable to human in their satellite images, but they have different class labels. Since the pretext task in contrastive learning is to maximize agreement between different views of the same image (positive pairs) and to minimize agreement between different images (negative pairs), high visual similarity across classes in the dataset might prevent the method from learning discriminative features.\chenlin{looks like our approach does not address this? because we are not modifying negative pair methods}
\s{expand a bit, you might need to explain a bit how contrastive methods work to give some intuition. typical contrastive  methods learn a featurization/embedding so that ... positive vs negative. this is needed anyways to contrast the typical approach to what you propose } \ayush{Done.}\chenlin{the contrastive method part is still not very clear}
%\burak{We can discuss why.}
\end{comment}

To bridge the gap between contrastive and supervised learning, we
% explore existing data augmentation methods for contrastive learning, and further 
propose geography-aware contrastive learning
%\chenlin{is "data augmentation methods" precise? that does not sound like self-supervised learning}
to leverage the spatio-temporal structure of remote sensing data. In contrast to typical computer vision images, remote sensing data are often geo-located
and might provide multiple images of the same location over time. 
%along with availability of temporal information (multiple images of the same location over time) that can be exploited.
% \s{unlike typical cv images, remote sensing data are almost always geo-located. there is also temporal structure that can be exploited, as we often get multiple images of the same location over time.}\ayush{Done}
%\s{unlike traditional .. where positive come from xxx, we }\ayush{Done.}
Unlike contrastive learning for traditional computer vision images where different views (augmentations) of the same image serve as a positive pair, our first improvement for remote sensing data comes from modifying
the contrastive learning objective to allocate \emph{temporal positive pairs} from spatially aligned images over time. Utilizing such information might allow the representations to incorporate subtle variations in locations over time thus resulting in more discriminative features useful for differentiating visually similar classes in the dataset.
%\s{why does this make sense intuitively? give intuition} \ayush{Done.}
Then, we design a novel unsupervised learning method, leveraging the geo-location information. 
\s{intuitively, just like patches from the same image are more likely to be semantically similar, images from locations that are close..}
This can be interpreted as predicting where in the world the image comes from similar to~\cite{hays2008im2gps,hays2015large}. Finally, we integrate the two proposed methods into the contrastive learning objective to shrink the gap with the supervised learning.

Our experiments on the functional Map of the World~\cite{christie2018functional} dataset consisting of high spatial resolution satellite images show that we improve MoCo-v2 baseline significantly. In particular, we improve it by $8\%$ classification accuracy when testing the learned representations
on image classification, $4\%$ AP on object detection, and $1\%$ mIoU on semantic segmentation. Interestingly, our geography-aware learning can even outperform the supervised learning counterpart on temporal data classification by $2\%$. To further demonstrate the effectiveness of our geography-aware learning approach, we extract the geo-location information of ImageNet images using FLICKR API similar to~\cite{de2019does}, which provides us with a subset of 543,435 geo-tagged ImageNet images. We extend the proposed approaches to geo-located ImageNet, and show that geography-aware learning can improve the performance of MoCo-v2 by $2\%$ on image classification, showing the potential application of our approach to any geo-tagged dataset. Figure~\ref{fig:approach} shows our contributions in detail.


==> sections/old.tex <==
% \chenlin{
% Contrastive learning~\cite{he2020momentum,chen2020simple,chen2020improved,tian2019contrastive,oord2018representation} is a framework that learns representations by contrasting semantically similar (positive) image pairs against dissimilar (negative) pairs. 
% % Recent progress on contrastive learning focuses on the design of contrastive loss, generation of positive and negative pairs, and sampling method. 
% In this work, we focus on the state-of-the-art contrastive learning framework MoCo-v2~\cite{chen2020improved}, an improved version of MoCo~\cite{he2020momentum} 
% and study the construction of positive and negative pairs.
% The contrastive loss function used in the MoCo-v2 framework is InfoNCE~\cite{oord2018representation}, which is defined as follows for a given data sample:
% % \begin{equation}
% % \footnotesize
% %   L = \mathbb{E}_{x_i, \hat{x}_{i}, \{k_j\}_{j=1}^{M}}\bigg[-\log \dfrac{\exp(z_{i}\cdot \hat{z}_{i}/\lambda)}{\exp(z_{i}\cdot\hat{z}_{i}/ \lambda) + \sum_{j=1}^{N}  \exp(z_{i}\cdot k_{j}/ \lambda)}\bigg],
% % \label{eq:moco}
% % \end{equation}
% % where $z_i$ is the encoded feature of $k_j$  represent the negative pairs of $z_i$, $N$ is size of negative samples per datapoint and $\lambda \in \mathbb{R}^{+}$ is the temperature hyperparameter.
% % need to define what z is, expectation should be over x 
% \begin{equation}
%   L_{z} = -\log \dfrac{\exp(z\cdot \hat{z}/\lambda)}{\exp(z\cdot \hat{z}/ \lambda) + \sum_{j=1}^{N}  \exp(z\cdot k_{j}/ \lambda)},
% \label{eq:moco}
% \end{equation}
% where $z$ is the encoded feature of the data sample, $N$ is number of negative samples, $\{k_j\}_{j=1}^{N}$ are the encoded negative pairs and $\lambda \in \mathbb{R}^{+}$ is the temperature hyperparameter.
% % In the case of the remote sensing, explain the input and output
% The key idea here is to encourage the encoding of positive pairs to have larger cosine similarity, and the encoding of negative pairs to have smaller cosine similarity.

% The construction of positive and negative pairs plays a crucial role in this framework. MoCo and MoCo-v2 both use perturbations (also called ``data augmentation") from the same image to create a positive sample. Commonly used perturbations include random color jittering, random horizontal flip, and random grayscale conversion.
% }

==> sections/old_.tex <==
\chenlin{
Unlike commonly seen natural image datasets
% like ImageNet~\cite{deng2009imagenet}
, remote sensing datasets often have extra temporal information, meaning that for a given location $(\textrm{lat}_i,\textrm{lon}_i)$, there exists
a sequence of images 
$\mathcal{X}_{i} = (x_i^1, \cdots, x_i^{T_i})$ taken over time at $(\textrm{lat}_i,\textrm{lon}_i)$. 
% A very special property of the temporal information is that 
Unlike in videos where nearby frames could experience huge content changes (\eg from a cat to a tree), the content of temporal information is often more stable across time. 
For instance, a place on ocean is likely to remain as ocean for months or years. In this case, satellite images taken at the same location should share high semantic similarities across time since all the images are about ocean.
Even for locations where changes do occur, certain semantic similarities could still remain. For instance, the same construction site is likely to have similar surroundings over time despite the ongoing construction. 

Given these observations, it is natural to leverage temporal information for remote sensing while constructing positive or negative pairs since it can provide us with extra semantically meaningful information of a place over time. More specifically, given an image $x_i^{t_1}$ collected at time $t_1$, we randomly select an image $x_i^{t_2}$ collected at the same location (\ie $x_i^{t_2}\in\mathcal{X}_{i}$). We then apply perturbations (\eg random color jittering) as used in MoCo-v2 to the two spatially aligned images $x_i^{t_1}$ and $x_i^{t_2}$, providing us with a \emph{temporal positive pair} that can be used for training the contrastive learning framework. Note that when $i=j$, the \emph{temporal positive pair} is the same as the positive pair used in MoCo-v2. We construct negative pairs by grouping two images with different geo-locations and then applying the same perturbations used in MoCo-v2 for constructing negative pairs.

Given a data sample $x_i^{t_1}$, our objective function can be formulated as follows:
\begin{equation}\small
  L_{z_i^{t_1}} = -\log \dfrac{\exp(z_{i}^{t_{1}}\cdot z_{i}^{t_{2}}/\lambda)}{\exp(z_{i}^{t_{1}}\cdot z_{i}^{t_{2}}/ \lambda) + \sum\limits_{j=1}^{N} \exp(z_{i}^{t_{1}}\cdot k_{j}/ \lambda)},
  \label{eq:temporal_positives}
\end{equation}
where $z_i^{t_1}$ is the encoded representation of $x_i^{t_1}$, and $z_i^{t_2}$ is the encoded representation of $x_i^{t_2}$, the temporal positive pair of $x_i^{t_1}$. Similar as \eqref{eq:moco}, $N$ is number of negative samples, $\{k_j\}_{j=1}^{N}$ are the encoded negative pairs and $\lambda \in \mathbb{R}^{+}$ is the temperature hyperparameter.
}

% We note that we do not change the negative pairs from the original objective in eq.~\ref{eq:moco}. In comparison to eq.~\ref{eq:moco} our main contribution is not solely relying on data augmentation to create positive pairs. We instead use two real images from the same area over time to create positives. We believe that relying on real images for positive pairs encourages the network to learn better representations for real data than the one relying on synthetic images for positive pairs.

% On the other hand, our objective in eq~\ref{eq:temporal_positives} enforces the representations to be invariant to changes over time. Depending on the target task, such inductive bias can be desirable or undesirable. For example, for a change detection task, learning representations that are variant to temporal changes can be more preferable. On the other hand, for image classification or object detection task, learning temporally invariant features should not degrade the downstream performance.
% In our experiments, we perform additional experiments on temporal data classification to analyze the usefulness of temporal positive pairs on this task.



% mention remote sensing has temporal info
% provide intuition:  ocean, and construction site

% how we construct positive negative pairs

% provide an equation

